TimeDiT: General-purpose Diffusion Transformers for Time Series Foundation Model

Foundation models, particularly Large Language Models (LLMs), have revolutionized text and video processing, yet time series data presents distinct challenges for such approaches due to domain-specific features such as missing values, multi-resolution characteristics, etc. Furthermore, the de-facto autoregressive transformers tend to learn deterministic temporal dependencies within pre-trained data while overlooking inherent uncertainties and lacking integration of physical constraints. In this paper, we introduce TimeDiT, a diffusion transformer model that synergistically combines transformer-based temporal dependency learning with diffusion-based probabilistic sampling. TimeDiT employs a unified masking mechanism to harmonize the training and inference process across diverse tasks while introducing a theoretically grounded, finetuning-free model editing strategy that enables flexible integration of external knowledge during sampling. Acknowledging the challenges of unifying multiple downstream tasks under a single model, our systematic evaluation demonstrates TimeDiT's effectiveness both in fundamental tasks, i.e., forecasting and imputation, through zero-shot/fine-tuning; and in domain tasks, i.e., multi-resolution forecasting, anomaly detection, and data generation, establishing it as a \textit{proto-foundation model} that bridges the gap between general-purpose and domain-specific models.

==> table/ETT.tex <==
\begin{table*}
  \centering
  \caption{Full results of long sequence forecasting experiments. Best results are highlighted in \textbf{bold}, and second best results are \underline{underlined}. Full-shot results are obtained from \cite{liu2023itransformer}.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{crcccccccccccccccccccccccc}
          \toprule
          &       & \multicolumn{8}{c}{\textbf{Zero-shot}}                 & \multicolumn{16}{c}{\textbf{Full-shot}} \\
          \cmidrule(lr){3-8} \cmidrule(lr){9-24}
          &  &\multicolumn{2}{c}{\textbf{TimeDiT}}     & \multicolumn{2}{c}{\textbf{{\smallmodel}}} & \multicolumn{2}{c}{\textbf{{\basemodel}}} & \multicolumn{2}{c}{\textbf{{\largemodel}}} & \multicolumn{2}{c}{\textbf{iTransformer}} & \multicolumn{2}{c}{\textbf{TimesNet}} & \multicolumn{2}{c}{\textbf{PatchTST}} & \multicolumn{2}{c}{\textbf{Crossformer}} & \multicolumn{2}{c}{\textbf{TiDE}} & \multicolumn{2}{c}{\textbf{DLinear}} & \multicolumn{2}{c}{\textbf{SCINet}} & \multicolumn{2}{c}{\textbf{FEDformer}} \\
          \midrule
          &     & \textbf{MSE} & \textbf{MAE}   & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} \\
          \midrule    \multirow{4}[1]{*}{ETTh1} & 96 & 0.325 & 0.386   & \textbf{0.375} & 0.402 & 0.384 & 0.402 & 0.380 & 0.398 & 0.386 & 0.405 & 0.384 & 0.402 & 0.414 & 0.419 & 0.423 & 0.448 & 0.479 & 0.464 & 0.386 & 0.400 & 0.654 & 0.599 & \underline{0.376} & 0.419 \\
          & 192 &0.347&0.390  & \textbf{0.399} & \textbf{0.419} & 0.425 & 0.429 & 0.440 & 0.434 & 0.441 & 0.436 & 0.436 & 0.429 & 0.460 & 0.445 & 0.471 & 0.474 & 0.525 & 0.492 & 0.437 & 0.432 & 0.719 & 0.631 & 0.420 & 0.448 \\
          & 336 & 0.347&0.396  & \textbf{0.412} & \textbf{0.429} & 0.456 & \underline{0.450} & 0.514 & 0.474 & 0.487 & 0.458 & 0.491 & 0.469 & 0.501 & 0.466 & 0.570 & 0.546 & 0.565 & 0.515 & 0.481 & 0.459 & 0.778 & 0.659 & 0.459 & 0.465 \\
          & 720 &0.404&0.440  & \textbf{0.413} & \textbf{0.444} & 0.470 & 0.473 & 0.705 & 0.568 & 0.503 & 0.491 & 0.521 & 0.500 & 0.500 & 0.488 & 0.653 & 0.621 & 0.594 & 0.558 & 0.519 & 0.516 & 0.836 & 0.699 & 0.506 & 0.507 \\
    \midrule
    \multirow{4}[0]{*}{ETTh2} & 96&0.257&0.331    & \underline{0.281} & 0.334 & \textbf{0.277} & 0.327 & 0.287 & 0.325 & 0.297 & 0.349 & 0.340 & 0.374 & 0.302 & 0.348 & 0.745 & 0.584 & 0.400 & 0.440 & 0.333 & 0.387 & 0.707 & 0.621 & 0.358 & 0.397 \\
          & 192 &0.316&0.380  & \underline{0.340} & 0.373 & \textbf{0.340} & 0.374 & 0.347 & 0.367 & 0.380 & 0.400 & 0.402 & 0.414 & 0.388 & 0.400 & 0.877 & 0.656 & 0.528 & 0.509 & 0.477 & 0.476 & 0.860 & 0.689 & 0.429 & 0.439 \\
          & 336 &0.341&0.418   & \textbf{0.362} & 0.393 & \underline{0.371} & 0.401 & 0.377 & 0.393 & 0.428 & 0.432 & 0.452 & 0.541 & 0.426 & 0.433 & 1.043 & 0.731 & 0.643 & 0.571 & 0.594 & 0.541 & 1.000 & 0.744 & 0.496 & 0.487 \\
          & 720 &0.447&0.441  & \textbf{0.380} & 0.416 & \underline{0.394} & 0.426 & 0.404 & 0.421 & 0.427 & 0.445 & 0.462 & 0.657 & 0.431 & 0.446 & 1.104 & 0.763 & 0.874 & 0.679 & 0.831 & 0.657 & 1.249 & 0.838 & 0.463 & 0.474\\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:lsf_full}%
\end{table*}%


==> table/ablation.tex <==
\begin{table*}[]
\centering
\begin{tabular}{llcccc}\toprule
          & Solar        & Electricity  & Traffic      & Taxi         & Exchange     \\ \hline
Attention & 0.095(0.002) & 0.015(0.001) & 0.266(0.003) & 0.196(0.003) & 0.168(0.009) \\
Add       & 0.091(0.001) & 0.021(0.000) & 0.136(0.002) & 0.201(0.004) & 0.206(0.006) \\
AdaLN     & 0.084(0.002) & 0.014(0.000) & 0.029(0.001) & 0.187(0.005) & 0.089(0.004)\\\bottomrule
\end{tabular}
\caption{Self-condition selection on observational data}
\end{table*}

==> table/forecasting.tex <==





\begin{table}[!t]
%\vspace{-0.15in}
\centering
\caption{Zero-shot Forecasting results on CRPS\_{sum}. Zero-shot implies that the model did not encounter any samples from the evaluating datasets during training.}
%\renewcommand{\arraystretch}{1.25}
%\resizebox{\textwidth}{!}{
\scalebox{0.8}{
\begin{tabular}{cccccc}\toprule
                        & \textbf{Solar}        & \textbf{Electricity}  & \textbf{Traffic}       & \textbf{Taxi }        & \textbf{Exchange}    \\ \hline 
        TEMPO& \underline{0.581(0.002)} & 0.081(0.003) & \underline{0.147(0.000)} & \underline{0.400(0.001)} & 0.030(0.001)\\
        Moirai(S) & 0.884(0.005) & 0.079(0.002) & 0.215(0.000) & 0.463(0.001) & \textbf{0.007(0.000)} \\
                   Moirai(B)  & 0.948(0.002) & 0.072(0.002) & 0.191(0.001) & 0.428(0.000) & 0.012(0.000) \\
                   Moirai(L) & 1.042(0.002) & \underline{0.039(0.001)} & \textbf{0.111(0.000)} & 0.597(0.000) & \underline{0.011(0.000)} \\
                   LagLLaMA     & 0.690(0.005) & 0.065(0.005) & 0.275(0.001) & 0.620(0.003) & 0.024(0.001) \\
                  TimeDiT         & \textbf{0.457(0.002)} & \textbf{0.026(0.001)} & 0.185(0.010) & \textbf{0.398(0.001)} & 0.021(0.002) \\ 

                   New - TimeDiT (S)        & \textbf{0.445(0.001)} & \textbf{0.030(0.001)} & - & \textbf{-} & 0.019(0.003) \\

                   New - TimeDiT (B)        & \textbf{0.640(0.006)} & \textbf{0.034(0.001)} & - & \textbf{-} & 0.040(0.004) \\

\bottomrule              
\end{tabular}

}
%\vskip -0.2in
\label{fore_zero}
\end{table}



